Semi-MapReduce Meets Congested Clique

Graph problems are troublesome when it comes to MapReduce. Typically, to be able to design algorithms that make use of the advantages of MapReduce, assumptions beyond what the model imposes, such as the density of the input graph, are required. In a recent shift, a simple and robust model of MapReduce for graph problems, where the space per machine is set to be O(|V|), has attracted considerable attention. We term this model semi-MapReduce, or in short, semiMPC, and focus on its computational power. We show through a set of simulation methods that semiMPC is, perhaps surprisingly, equivalent to the congested clique model of distributed computing. However, semiMPC, in addition to round complexity, incorporates another practically important dimension to optimize: the number of machines. Furthermore, we show that algorithms in other distributed computing models, such as CONGEST, can be simulated to run in the same number of rounds of semiMPC while also using an optimal number of machines. We later show the implications of these simulation methods by obtaining improved algorithms for these models using the recent algorithms that have been developed.

==> packages.tex <==
\usepackage{amsmath, amsthm, amssymb}
\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{mathtools}
\usepackage{comment} % enables comment environment
\usepackage{color-edits} % author comments with colors
\usepackage{tcolorbox}
\usepackage{xfrac}
\usepackage{hyperref}
\usepackage{multirow}

==> proofs.tex <==




==> summary.tex <==
We start with the formal definition of the {\em massively parallel communications} model which was first introduced in \cite{beame2013communication}.

\negspace{}
\paragraph{The \MPC{} model.} An input (not necessarily a graph) of size $\ell$ is initially distributed among $p$ machines (processors) each with a space of size $s$. The total space of all machines (i.e., $p \cdot s$) is bounded by $\Ot{\ell ^ {1 + \delta}}$ for a small parameter $\delta \in [0, 1)$ of the algorithm that controls \emph{replication}. Furthermore, the number of machines should not be more than the space per machine\footnote{This is motivated by a practical restriction that each machine should be able to store the identifier (e.g., IP) of all other machines to be able to communicate with them.} (i.e., $p \leq s$). Computation proceeds in synchronous \emph{rounds}: In each round, each machine performs a local computation on its data, and at the end of the round, communicates with other machines. The total size of the messages that a machine sends or receives in each round should not be more than its space $s$.

We are now ready to formalize \semiMPC{} for graph problems.

\negspace{}
\paragraph{The \semiMPC{} model.} Let $G = (V, E)$ with $n = |V|$ and $m = |E|$, be the input graph. An algorithm is in \semiMPC{} if it is in \MPC{} and each machine uses a space of $\O{n}$ words.

\begin{theorem} \label{thm:cc-mpc}
	Let $\mathcal{A}_{CC}$ be an algorithm that for an input graph $G=(V, E)$, with $n$ vertices, runs in $T$ rounds of \CC{} using a local memory of $\O{n}$ in each node. One can simulate $\mathcal{A}_{CC}$ in $\O{T}$ rounds of \semiMPC{} using $n$ machines.
\end{theorem}

\begin{theorem}\label{thm:mpc-cc}
	Let $\mathcal{A}_M$ be an algorithm that for an input graph $G$, with $n$ vertices, runs in $T$ rounds of \semiMPC{}. One can simulate $\mathcal{A}_M$ in $\O{T}$ rounds of \CC{}.
\end{theorem}

\begin{theorem}\label{thm:congest-mpc}
	Let $\mathcal{A}_C$ be an algorithm that for an input graph with $n$ vertices and $m$ edges runs in $T$ rounds of \CONGEST{} while using, on each node, a local memory that is linear in the total messages that it receives. One can simulate $\mathcal{A}_C$ in $T$ rounds of \semiMPC{} using at most $\O{T \cdot m/n}$ machines.
\end{theorem}

\negspace{}\negspace{}
\paragraph{Implications.} These simulation methods, while not hard to prove, have significant consequences. For instance, by combining the recent algorithm of Jurdzi\'{n}ski and Nowicki \cite{jurdzinski2018mst} and Theorem~\ref{thm:cc-mpc}, we obtain the following which improves prior connectivity and MST algorithms on \semiMPC{} and \MPC{}. \cite{lattanzi2011filtering, bateni2017affinity}
\negspace{}
\begin{corollary}
	There exists an $\O{1}$ round algorithm for computing the minimum spanning tree and graph connectivity on \semiMPC{}.
\end{corollary}
\negspace{}
Furthermore, by combining the recent approximate maximum matching algorithm of Czumaj \etal{}~\cite{czumaj2017round} and Theorem~\ref{thm:mpc-cc} we get the first sub-logarithmic round algorithm of this problem for the congested clique.
\negspace{}

\sbcomment{Update with assadi}
\begin{corollary}
	There exists an $\O{\log^2 \log n}$ round algorithm for computing an $\O{1}$ approximate maximum matching on the congested clique.
\end{corollary}

\sbcomment{Add vertex cover.}






